Improving Both Domain Robustness and Domain Adaptability in Machine Translation

We consider two problems of NMT domain adaptation using meta-learning. First, we want to reach domain robustness, i.e., we want to reach high quality on both domains seen in the training data and unseen domains. Second, we want our systems to be adaptive, i.e., making it possible to finetune systems with just hundreds of in-domain parallel sentences. We study the domain adaptability of meta-learning when improving the domain robustness of the model. In this paper, we propose a novel approach, RMLNMT (Robust Meta-Learning Framework for Neural Machine Translation Domain Adaptation), which improves the robustness of existing meta-learning models. More specifically, we show how to use a domain classifier in curriculum learning and we integrate the word-level domain mixing model into the meta-learning framework with a balanced sampling strategy. Experiments on English$\rightarrow$German and English$\rightarrow$Chinese translation show that RMLNMT improves in terms of both domain robustness and domain adaptability in seen and unseen domains. Our source code is available at https://github.com/lavine-lmu/RMLNMT.

==> Makefile <==
SHELL=bash
NAME=acl_latex
LATEX=pdflatex
FILES=$(NAME).tex custom.bib anthology.bib

all: $(NAME).pdf

$(NAME).pdf: $(FILES)
	latexmk -pdflatex="$(LATEX) %O %S" -pdf -dvi- -ps- -halt-on-error $(NAME)

watch:
	latexmk -pdflatex="$(LATEX) %O %S" -pdf -dvi- -ps- -interaction=nonstopmode -synctex=1 -pvc $(NAME)

view:
	xdg-open $(NAME).pdf

force: $(NAME).tex references.bib scheme.tex
	latexmk -pdflatex="$(LATEX) %O %S" -pdf -dvi- -ps- $(NAME)

clean:
	rm -f $(NAME).{aux,bbl,log,out,pdf}
	rm -r html

.PHONY: html
html: $(FILES)
	mkdir -p html
	sed -e 's/\\input{/\\fbox{INPUT: /;s/\\pdfoutput.*//' $(NAME).tex > main_html.tex
	make4ht -e mk4ht.mk4 --xetex --utf8 --jobname $(NAME)_html --output-dir html $(NAME)_html.tex
	bibtex $(NAME)_html
	make4ht -e mk4ht.mk4 --xetex --utf8 --jobname $(NAME)_html --output-dir html $(NAME)_html.tex
	rm $(NAME)_html-*.{svg,png} $(NAME)_html*.* || true

